Learning Realistic Traffic Agents in Closed-loop

Realistic traffic simulation is crucial for developing self-driving software in a safe and scalable manner prior to real-world deployment. Typically, imitation learning (IL) is used to learn human-like traffic agents directly from real-world observations collected offline, but without explicit specification of traffic rules, agents trained from IL alone frequently display unrealistic infractions like collisions and driving off the road. This problem is exacerbated in out-of-distribution and long-tail scenarios. On the other hand, reinforcement learning (RL) can train traffic agents to avoid infractions, but using RL alone results in unhuman-like driving behaviors. We propose Reinforcing Traffic Rules (RTR), a holistic closed-loop learning objective to match expert demonstrations under a traffic compliance constraint, which naturally gives rise to a joint IL + RL approach, obtaining the best of both worlds. Our method learns in closed-loop simulations of both nominal scenarios from real-world datasets as well as procedurally generated long-tail scenarios. Our experiments show that RTR learns more realistic and generalizable traffic simulation policies, achieving significantly better tradeoffs between human-like driving and traffic compliance in both nominal and long-tail scenarios. Moreover, when used as a data generation tool for training prediction models, our learned traffic policy leads to considerably improved downstream prediction metrics compared to baseline traffic agents. For more information, visit the project website: https://waabi.ai/rtr

==> figures/merged_1.tex <==

\begin{wrapfigure}[11]{r}{0.67\textwidth}
    % \begin{figure}[t]
    \vspace{-10pt}
    \begin{floatrow}
        % \capbtabbox[0.25\textwidth]{%
        \capbtabbox[0.37\textwidth]{%
            \small
            \begin{tabular}{@{}lcc@{}}
                \toprule
                Method                   & Col.          & FDE           \\
                \cmidrule(r){1-1} \cmidrule(lr){2-3}
                % GT   &  & &  & & &\\
                BC                       & 8.70          & 2.40          \\
                IL                       & 8.40          & 1.80          \\
                RL                       & 5.41          & 16.89         \\
                RL-Shp                   & 5.95          & 6.80          \\
                BC+RL                    & \textbf{5.15} & 9.30          \\
                \rowcolor{grey}\ourmodel & 7.29          & \textbf{1.57} \\ \bottomrule
            \end{tabular}
        }{%
            \caption{\ourmodel{} generates better data for training.}
            \label{tab:downstream}
        }
        % \capbtabbox[0.38\textwidth]{%
        \capbtabbox[0.63\textwidth]{%
            \small
            \centering
            \begin{tabular}{@{}ccccc|c@{}}
                \toprule
                          &          & \multicolumn{3}{c|}{Nominal} & LT                                            \\
                $\lambda$ & $\alpha$ & Col.                         & FDE           & Acc.          & Col.          \\
                \cmidrule(r){1-2} \cmidrule(lr){3-5} \cmidrule(l){6-6}
                1.0       & 0.5      & 0.38                         & 5.50          & 0.18          & 3.61          \\
                5.0       & 0.5      & 0.38                         & 5.16          & \textbf{0.16} & 3.61          \\
                10        & 0.5      & 0.52                         & \textbf{5.10} & 0.17          & 3.82          \\
                5.0       & 0.3      & \textbf{0.35}                & 5.20          & 0.17          & 4.12          \\
                5.0       & 0.7      & 0.56                         & 6.10          & 0.23          & \textbf{3.51} \\
                \bottomrule
            \end{tabular}
        }{%
            \caption{Balancing the trade-off between realism and infraction avoidance of \ourmodel{}.}
            \label{tab:balancing}
        }
    \end{floatrow}
\end{wrapfigure}
% \end{figure}

==> figures/scenario_sets.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
    \includegraphics[width=0.98\columnwidth]{assets/scenario_sets.pdf}
    \caption{Using both nominal and long-tail yields the best tradeoff.}
    % \simon{Here we introduce yet another collision rate (Curated Col.)
    % I think the differences are too nuanced and hard to keep track for reader. 
    % I'd recommend removing the plot or show something else.}
    \label{fig:scenario_sets}
\end{wrapfigure}


==> figures/teaser.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
    \centering
    \includegraphics[width=0.48\textwidth]{assets/teaser_v6.pdf}
    \caption{
    %Our multi-agent actor policy is trained using imitation learning (IL) and reinforcement learning (RL) in a closed-loop environment. 
    Learning multi-agent policies for traffic simulation in closed-loop. 
    IL leverages real data while   
    RL explicitly penalizes infractions like collision. 
    Since RL does not require expert demonstration, it can learn from additional procedurally generated long-tail scenarios.}
\label{fig:teaser}
\end{wrapfigure}


==> figures/training_curve.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \vspace{-5pt}
    \includegraphics[width=0.49\textwidth]{assets/training_curve_collision.pdf}
    \includegraphics[width=0.49\textwidth]{assets/training_curve_offroad.pdf}
    \caption{Comparing our factorized PPO compared to standard PPO
        which uses a single scene-level reward.}\label{fig:training_curve}
\end{wrapfigure}

==> tables/hard_table.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{@{}ccccccccc@{}}
        \toprule
        \multicolumn{3}{c}{Train Data}   & \multicolumn{3}{c}{Nominal}                 & \multicolumn{2}{c}{Curated}     & SC \\ 
        N        & H        & SC         & Col.            & Off.            & FDE           & CR            & OR            & Col.            \\ 
            \cmidrule(r){1-3}      \cmidrule(lr){4-6}                           \cmidrule(lr){7-8}                 \cmidrule(l){9-9}
        \checkmark &            &            & 0.38 & 0.49          & 5.05 & 0.83          & 1.09          & 9.60          \\
                   & \checkmark &            & 0.45          & 0.14          & 5.34          & 0.88          & 0.32          & 9.42          \\
        & & \checkmark           &         0.58 &   0.48 &    6.26 &     1.27 &     1.05 &     4.00      \\
        \checkmark &            & \checkmark & 0.38 & 0.20          & 5.16          & 0.85          & 0.45          & 3.61 \\ \bottomrule
        \end{tabular}
    \caption{Comparing train and eval of different scenario datasets. Maybe can be in appendix as we have Figure 6 which tells story better.}
    \label{tab:hard}
\end{table}
